Generating Signed Permutations by Twisting Two-Sided Ribbons

We provide a simple and natural solution to the problem of generating all $2^n \cdot n!$ signed permutations of $[n] = \{1,2,\ldots,n\}$. Our solution provides a pleasing generalization of the most famous ordering of permutations: plain changes (Steinhaus-Johnson-Trotter algorithm). In plain changes, the $n!$ permutations of $[n]$ are ordered so that successive permutations differ by swapping a pair of adjacent symbols, and the order is often visualized as a weaving pattern involving $n$ ropes. Here we model a signed permutation using $n$ ribbons with two distinct sides, and each successive configuration is created by twisting (i.e., swapping and turning over) two neighboring ribbons or a single ribbon. By greedily prioritizing $2$-twists of the largest symbol before $1$-twists of the largest symbol, we create a signed version of plain change's memorable zig-zag pattern. We provide a loopless algorithm (i.e., worst-case $\mathcal{O}(1)$-time per object) by extending the well-known mixed-radix Gray code algorithm.

==> unused/greedyAlgs.tex <==
% different ways of writing the greedy algorithm


\begin{algorithm}[h]
\centering
\caption{A greedy algorithm for generating twisted plain changes.}
\label{alg:greedy}
\begin{algorithmic}[1]
\Statex $\AlgGreedy{n}$
\State $T \leftarrow \twtLeft{n}, \twtRight{n}, \ldots, \twtLeft{2}, \twtRight{2}, \twtRight{1}, \twtLeft{1}, \; \twt{n}, \ldots, \twt{2}, \twt{1}$ \Comment{List of $3n$ different twists}
\State $i \leftarrow 1$ \Comment{1-based index into $T$ (e.g., $T[1]$ is $\twtLeft{n}$)}
\State $\pi \leftarrow {+}1 \ {+}2 \ \cdots \ {+}n$ \Comment{Starting signed permutation $\pi \in \SIGNED{n}$}
\State $\Visit{\pi}$ \Comment{Visit $\pi$ for the first and only time}
\State $S = \{\pi\}$ \Comment{Add $\pi$ to the visited set}
\While{$i \leq 3n$} \Comment{Index $i$ iterates through the $3n$ different twists}
  \State $\pi' \leftarrow T[i](\pi)$ \Comment{Apply the $i^{\text{th}}$ highest priority twist to create $\pi'$}
  \If{$\pi' \notin S$} \Comment{Check if $\pi'$ is a new signed permutation}
    \State $\pi \leftarrow \pi'$ \Comment{Update the current signed permutation $\pi$}
    \State $\Visit{\pi}$ \Comment{Visit $\pi$ for the first and only time}
    \State $S = S \cup \{\pi\}$ \Comment{Add $\pi$ to the visited set}
    \State $i \leftarrow 1$ \Comment{Reset the 1-based index into $T$}
  \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\centering
\caption{A greedy algorithm for generating twisted plain changes.}
\label{alg:greedy}
\begin{algorithmic}[1]
\Statex $\AlgGreedy{n}$
\State $\pi \leftarrow {+}1 \ {+}2 \ \cdots \ {+}n$ \Comment{Create the first $\pi \in \SIGNED{n}$}
\State $\Visit{\pi}$ \Comment{Visit $\pi$}
\State $S = \{\pi\}$ \Comment{Add $\pi$ to the visited set}
\State $C \leftarrow \twitLeft{\pi}{n}, \twitRight{\pi}{n}, \ldots, \twitRight{\pi}{1}, \twitLeft{\pi}{1}, \twit{\pi}{n}, \ldots, \twit{\pi}{1}$ \Comment{Prioritized list of candidates}
\State $i \leftarrow 1$
\While{$i \leq 3n$} \Comment{Iterator over the candidates}
  \State $\pi' = C[i]$
  \If{$\pi' \notin S$}
    \State $\pi \leftarrow \pi'$
    \State $\Visit{\pi'}$
    \State $S = S \cup \{\pi\}$
    \State $C \leftarrow \twitLeft{\pi}{n}, \twitRight{\pi}{n}, \ldots, \twitRight{\pi}{1}, \twitLeft{\pi}{1}, \twit{\pi}{n}, \ldots, \twit{\pi}{1}$ \Comment{Candidates}
    \State $i \leftarrow 1$
  \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\centering
\caption{A greedy algorithm for generating twisted plain changes.}
\label{alg:greedy}
\begin{algorithmic}[1]
\Statex $\AlgGreedy{n}$
\State $\pi \leftarrow {+}1 \ {+}2 \ \cdots \ {+}n$
\State $\Visit{\pi}$
\State $i \leftarrow 1$
\While{$i \leq 3 \cdot n$}
  \Comment{Apply the $i$th priority modification to create the candidate $\pi'$}
  \If{$i \leq 2n$ and $i \mod 2 = 1$}
    \State $\pi' \leftarrow \twistLeft{\pi}{i}$
  \ElsIf{$i \leq 2n$ and $i \mod 2 = 0$}
    \State $\pi' \leftarrow \twistLeft{\pi}{i}$
  \Else
    \State $\pi' \leftarrow \twist{\pi}{i}$
  \EndIf
  \State $i \leftarrow i+1$
  \Comment{Check if the candidate is new}
  \If{$\pi' \notin S$}
    \State $\pi \leftarrow \pi'$
    \State $\Visit{\pi}$
    \State $i \leftarrow 1$
  \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

% 
\begin{algorithm}[h]
\centering
\caption{A greedy algorithm for generating twisted plain changes.}
\label{alg:greedy}
\begin{algorithmic}[1]
\Statex $\AlgGreedy{n}$
\State $\pi \leftarrow {+}1 \ {+}2 \ \cdots \ {+}n$ \Comment{Create the first object $\pi$}
\State $\Visit{\pi}$ \Comment{Visit the first object}
\LineComment{Create the list of candidates}
\State $C \leftarrow \twistLeft{\pi}{n}, \twistRight{\pi}{n}, \ldots, \twistRight{\pi}{1}, \twistLeft{\pi}{1}, \twist{\pi}{n}, \ldots, \twist{\pi}{1}$
\For{$\pi' \in C$}
  \If{$\pi' \notin S$}
    \State $\pi \leftarrow \pi'$
    \State $\Visit{\pi'}$
    \State $C \leftarrow \twistLeft{\pi}{n}, \twistRight{\pi}{n}, \ldots, \twistRight{\pi}{1}, \twistLeft{\pi}{1}, \twist{\pi}{n}, \ldots, \twist{\pi}{1}$
  \EndIf
\EndFor
\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[h]
% \centering
% \caption{A greedy algorithm for generating twisted plain changes.}
% \label{alg:greedy}
% \begin{algorithmic}[1]
% \Statex $\AlgGreedy{n}$
% \State $\pi \leftarrow {+}1 \ {+}2 \ \cdots \ {+}n$
% \State $\Visit{\pi}$
% \State $j \leftarrow n$
% \State $i \leftarrow n$
% \While{$j \geq 1$}
%   \While{$i \geq 1$}
%     \If{$twistLeft(\pi,i) \notin S$} 
%       \State $\pi \leftarrow twistLeft(\pi,i)$ 
%       \State $\Visit{\pi}$
%       \State $i \leftarrow n$
%     \ElsIf{$twistRight(\pi,i) \notin S$} 
%       \State $\pi \leftarrow twistRight(\
